IRLab@iKAT24: Learned Sparse Retrieval with Multi-aspect LLM Query Generation for Conversational Search

The Interactive Knowledge Assistant Track (iKAT) 2024 focuses on advancing conversational assistants, able to adapt their interaction and responses from personalized user knowledge. The track incorporates a Personal Textual Knowledge Base (PTKB) alongside Conversational AI tasks, such as passage ranking and response generation. Query Rewrite being an effective approach for resolving conversational context, we explore Large Language Models (LLMs), as query rewriters. Specifically, our submitted runs explore multi-aspect query generation using the MQ4CS framework, which we further enhance with Learned Sparse Retrieval via the SPLADE architecture, coupled with robust cross-encoder models. We also propose an alternative to the previous interleaving strategy, aggregating multiple aspects during the reranking phase. Our findings indicate that multi-aspect query generation is effective in enhancing performance when integrated with advanced retrieval and reranking models. Our results also lead the way for better personalization in Conversational Search, relying on LLMs to integrate personalization within query rewrite, and outperforming human rewrite performance.

==> tables/main_res_sub.tex <==
\begin{table*}[t]
\centering
\caption{Experimental results on the official evaluation set. Bold indicates the best results and \textit{italic} shows the best results between Automatic runs.}
\label{tab:main_tab}
\resizebox{1.1\textwidth}{!}{
\begin{tabular}{l|l|l|cccc}
\midrule
% \hline
\textbf{Runs} & \textbf{LLM} &\textbf{Reranker} & \textbf{nDCG@5} & \textbf{nDCG} & \textbf{MRR} & \textbf{R@100}\\ 
\midrule
(1) MQ4CS-QR & GPT4  & DebertaV3 & \textbf{0.5213} & 0.6098 & 0.8479 & 0.4366 \\ 
(2) MQ4CS-QR & GPT4  & Ensemble & 0.5155 & \textbf{0.6192} & \textbf{0.8644} & \textbf{0.4657} \\ 
(3) GPT4QR & GPT4  & DebertaV3 & 0.5071 & 0.5420 & 0.8315 & 0.4135  \\ 
% (4) GPT4QR-bm25-QD1 & GPT4 & BM25 & MiniLM & 0.4768 & 0.4373 & 0.8476 & 0.3421 & 0.5199 & 0.2315 \\ 
\midrule
(5) HumanQR &Human & DebertaV3 & 0.4767 & 0.5496 & 0.7808 & 0.4263   \\
(6) HumanQR &Human & Ensemble & 0.5384 & 0.5819 & 0.8483 & 0.4777   \\ 
% \hline
\midrule
% \midrule
% \textbf{Run Manual} & \textbf{LLM}& \textbf{Retrieval} & \textbf{Reranker} & \textbf{nDCG@5} & \textbf{nDCG} & \textbf{MRR} & \textbf{Recall@100} & \textbf{P@20} & \textbf{mAP} \\ 
% \midrule
% HumanQR-deberta &Human& SPLADE & DebertaV3 & 0.4767 & 0.5496 & 0.7808 & 0.4263 & 0.5383 & 0.3072 \\
% HumanQR-ensemble &Human& SPLADE & Ensemble & 0.5384 & 0.5819 & 0.8483 & 0.4777 & 0.5922 & 0.3533 \\ 
% \hline
\end{tabular}
}
\end{table*}
